Generalizable Decision Boundaries: Dualistic Meta-Learning for Open Set Domain Generalization

Domain generalization (DG) is proposed to deal with the issue of domain shift, which occurs when statistical differences exist between source and target domains. However, most current methods do not account for a common realistic scenario where the source and target domains have different classes. To overcome this deficiency, open set domain generalization (OSDG) then emerges as a more practical setting to recognize unseen classes in unseen domains. An intuitive approach is to use multiple one-vs-all classifiers to define decision boundaries for each class and reject the outliers as unknown. However, the significant class imbalance between positive and negative samples often causes the boundaries biased towards positive ones, resulting in misclassification for known samples in the unseen target domain. In this paper, we propose a novel meta-learning-based framework called dualistic MEta-learning with joint DomaIn-Class matching (MEDIC), which considers gradient matching towards inter-domain and inter-class splits simultaneously to find a generalizable boundary balanced for all tasks. Experimental results demonstrate that MEDIC not only outperforms previous methods in open set scenarios, but also maintains competitive close set generalization ability at the same time. Our code is available at https://github.com/zzwdx/MEDIC.

==> figs/boundary.tex <==
\begin{figure*}[tp]
   
    \centering
    \includegraphics[width=0.95\linewidth]{pictures/boundary.jpg}
    \caption{An example for the variation of prediction probability in open set domain generalization.}
    \vspace{-0.15in}
    \label{fig:boundary}
\end{figure*}

==> figs/conf_cmp.tex <==
\begin{figure}[tp]
    \centering
    \hspace{-0.04\linewidth}
	\begin{subfigure}{0.51\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{pictures/conf_cmp_abs.jpg}
		\label{subfig:conf_cmp_abs}
	\end{subfigure}
    \vspace{0in}
	\begin{subfigure}{0.51\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{pictures/conf_cmp_rel.jpg}
		\label{subfig:conf_cmp_rel}
	\end{subfigure}
    
	\vspace{-0.15in}
	\caption{Comparison of absolute (\emph{Left}) and relative (\emph{Right}, subtracting domain-wise) confidence on unknown target samples between different matching patterns in descending order (lower is better).}
    \vspace{-0.18in}
    
	\label{fig:conf_cmp}
\end{figure}

==> figs/split.tex <==
\begin{figure}[tp]
    \centering
    \vspace{-0.1in}
    %\hspace{-0.1\linewidth}
    \includegraphics[width=1\linewidth]{pictures/match.jpg}
    \vspace{-0.2in}
    \caption{
    Insights of \todo{}.
    The black arrows indicate the matching patterns from current meta-learning-based DG methods, while we attempt to fill their gap at the category level. 
    }
    \vspace{-0.2in}
    \label{fig:match}
\end{figure}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> sections/11_acknowledgement.tex <==
\section*{Acknowledgement}
\label{sec:ackownledgement}
This work was supported by NSFC Major Program (62192783), CAAI-Huawei MindSpore Project (CAAIXSJLJJ-2021-042A), China Postdoctoral Science Foundation Project (2021M690609), Jiangsu Natural Science
Foundation Project (BK20210224), and CCF-Lenovo Bule Ocean Research Fund.
